Neural Network Compression of ACAS Xu Early Prototype is Unsafe: Closed-Loop Verification through Quantized State Backreachability

ACAS Xu is an air-to-air collision avoidance system designed for unmanned aircraft that issues horizontal turn advisories to avoid an intruder aircraft. Due the use of a large lookup table in the design, a neural network compression of the policy was proposed. Analysis of this system has spurred a significant body of research in the formal methods community on neural network verification. While many powerful methods have been developed, most work focuses on open-loop properties of the networks, rather than the main point of the system -- collision avoidance -- which requires closed-loop analysis. In this work, we develop a technique to verify a closed-loop approximation of the system using state quantization and backreachability. We use favorable assumptions for the analysis -- perfect sensor information, instant following of advisories, ideal aircraft maneuvers and an intruder that only flies straight. When the method fails to prove the system is safe, we refine the quantization parameters until generating counterexamples where the original (non-quantized) system also has collisions.

==> apx_ah_polytopes.tex <==
\section{$\mathcal{AH}$-Polytopes: Formal Definition and Operations}
\label{apx:ahpoly}
The $\mathcal{AH}$-Polytope representation is informally an affine trasnformation of a half-space polytope, where the affine transformation and polytope are kept explicitly separate.
%
This representation is extremely useful for reachability of continuous and hybrid systems with linear dynamics.
%
The name was introduced fairly recently~\cite{sadraddini2019linear}, although it has been regularly used for hybrid systems reachability analysis as well as neural network verification.
%
Here, we provide a formal definition and list key set operations for the representations used in our approach.

%\textcolor{red}{An $\mathcal{AH}$-Polytope is a tuple $\Theta = \langle V, c, C, d \rangle$ that represents a set of states as follows
%$\llbracket \Theta \rrbracket = \{x \in \mathbb{R}^n ~ | ~ \exists_{\alpha \in \mathbb{R}^m} ~ x = V \alpha + c \wedge C\alpha \leq d \}$
%
%We generally refer to both the tuple $\Theta$ and the set of states $\llbracket \Theta \rrbracket$ as $\Theta$ as it is clear from context which one we are referring to.
%
%(Maybe you can change some of the letters or parts to make this cleaner?)}

%Star Set Representation
%We present briefly the definition and some important properties of a star set used in the proposed backward reachability.
%
\begin{definition} [$\mathcal{AH}$-Polytope] \label{def:AH-polytope} An $\mathcal{AH}$-Polytope is a tuple $\Theta = \langle V, c, C, d \rangle$ that represents a set of states as follows:
\begin{equation*}
 \llbracket \Theta \rrbracket = \{x \in \mathbb{R}^n ~ | ~ \exists {\alpha \in \mathbb{R}^m}, ~ x = V \alpha + c \wedge C\alpha \leq d\}.   
\end{equation*}
\end{definition}
We generally refer to both the tuple $\Theta$ and the set of states $\llbracket \Theta \rrbracket$ as $\Theta$ as it is clear from context which one we are referring to.
%
\begin{proposition}[Affine Mapping] An affine mapping of an $\mathcal{AH}$-Polytope $\Theta = \langle V, c, C, d \rangle$ with a mapping matrix $W$ and an offset vector $b$ is a new $\mathcal{AH}$-Polytope $\Theta^\prime = \langle V^\prime, c^\prime, C^\prime, d^\prime \rangle$ in which $V^\prime = WV,~c^\prime = Wc + b,~C^\prime = C,~d^\prime = d$.
\end{proposition}
%
\begin{proposition}[Linear Transformation] A linear transformation of an $\mathcal{AH}$-Polytope with a matrix $W$ is an affine mapping using mapping matrix $W$ and an offset vector of $b = 0$.
\end{proposition}
%
\begin{proposition}[Intersection] The intersection of $\Theta = \langle V, c, C, d \rangle$ and a half-space $\mathcal{H} = \{x~|~Gx \leq g \}$ is a new $\mathcal{AH}$-Polytope $\Theta^\prime = \langle V^\prime, c^\prime, C^\prime, d^\prime \rangle $ with $c^\prime = c,~V^\prime = V,~C^\prime = [C;GV],~d^\prime = [d;g-Gc]$.
\end{proposition}
%
\begin{proposition}[Linear Optimization] Linear optimization in given a direction $w \in \mathbb{R}^n$ over a star set
%
$\Theta = \langle V, c, C, d \rangle$
%
can be solved with linear programming as follows:
%
$min(w^T x), ~s.t.~ x \in \Theta = 
w^T c + min(w^T V \alpha),~s.t.~C\alpha \leq d$.
\end{proposition}
